Advanced Bloom Filter Based Algorithms for Efficient Approximate Data De-Duplication in Streams

Applications involving telecommunication call data records, web pages, online transactions, medical records, stock markets, climate warning systems, etc., necessitate efficient management and processing of such massively exponential amount of data from diverse sources. De-duplication or Intelligent Compression in streaming scenarios for approximate identification and elimination of duplicates from such unbounded data stream is a greater challenge given the real-time nature of data arrival. Stable Bloom Filters (SBF) addresses this problem to a certain extent. . In this work, we present several novel algorithms for the problem of approximate detection of duplicates in data streams. We propose the Reservoir Sampling based Bloom Filter (RSBF) combining the working principle of reservoir sampling and Bloom Filters. We also present variants of the novel Biased Sampling based Bloom Filter (BSBF) based on biased sampling concepts. We also propose a randomized load balanced variant of the sampling Bloom Filter approach to efficiently tackle the duplicate detection. In this work, we thus provide a generic framework for de-duplication using Bloom Filters. Using detailed theoretical analysis we prove analytical bounds on the false positive rate, false negative rate and convergence rate of the proposed structures. We exhibit that our models clearly outperform the existing methods. We also demonstrate empirical analysis of the structures using real-world datasets (3 million records) and also with synthetic datasets (1 billion records) capturing various input distributions.

==> proof.tex <==
%\documentclass{sig-alternate}
%\usepackage[utf8x]{inputenc}

%\usepackage{times}
%\usepackage{amsmath}
%\usepackage{amsthm}
%\newtheorem{theorem}{Theorem}[section]

\section{General Framework}
\label{framework}
We first present a generic framework for analyzing the false positive rate (FPR) and false negative rate (FNR) of our algorithms. In fact this framework can be used for FPR and FNR analysis of any Bloom Filter based algorithms. A false positive (FP) event occurs if a distinct element of the stream is reported as duplicate. A false negative (FN) event occurs when a duplicate element of the stream is reported as distinct.

Now we consider the scenario under which FP or FN can take place. Assume $e_{m+1}$, the $(m+1)^{th}$ element of the stream has arrived. Let $e_{m+1}$ hashes to $H_{m+1}={h_1,h_2,...,h_k}$ positions where $h_i \in [1,s]$ for the $i^{th}$ Bloom Filter. $e_{m+1}$ will be reported as a duplicate by the algorithm if all the bit positions in $H_{m+1}$ are set to $1$. Let $X_{m+1}$ be the probability of this event. If at least one of the bit positions in $H_{m+1}$ is $0$, then $e_{m+1}$ will be reported as distinct.  Also let us denote by $Y_{m+1}$ the probability that $e_{m+1}$ is actually a distinct element. So to begin with we have:
\begin{align}
X_{m+1} &= P(\text{all bit posotions in $H_{m+1}$ are $1$ when $e_{m+1}$ arrived})\\
Y_{m+1} &= P(\text{$e_{m+1}$ is actually a distinct element})
\end{align}

Now using $X_{m+1}$ and $Y_{m+1}$ we can determine the probability that $e_{m+1}$ will result in a FP or FN. Assume $FPR_{m+1}$ and $FNR_{m+1}$ denotes the probability that ${m+1}^{th}$ element of the stream is a FP and FN respectively. So
\begin{align}
FPR_{m+1}&= P(\text{$e_{m+1}$ is actually distinct}).P(\text{$e_{m+1}$ is reported duplicate}) \nonumber\\
&= P(\text{$e_{m+1}$ is actually distinct}).P(\text{all bit posotions in $H_{m+1}$} \nonumber \\
& \qquad \qquad\text{are $1$ when $e_{m+1}$ arrived}) \nonumber \\
&= Y_{m+1}.X_{m+1} \\		
FNR_{m+1}&= P(\text{$e_{m+1}$ is actually a duplicate}).P(\text{$e_{m+1}$ is reported distinct}) \nonumber\\
&= P(\text{$e_{m+1}$ is actually a duplicate}).P(\text{not all bit positions in} \nonumber \\
& \qquad \qquad \text{$H_{m+1}$ are $1$ when $e_{m+1}$ arrived}) \nonumber\\
&= (1-Y_{m+1}).(1-X_{m+1})
\end{align}

For simplicity of analysis, we consider the probability of two more events: (i) the algorithm correctly predicts $e_{m+1}$ as duplicate, (ii) the algorithm correctly predicts $e_{m+1}$ as distinct. Let us denote by $DUP_{m+1}$ and $DIS_{m+1}$ the probability of the event (i)and event (ii) respectively. Then we can derive the expression for $DUP_{m+1}$ and $DIS_{m+1}$ as follows:
\begin{align}
DUP_{m+1}&= P(\text{$e_{m+1}$ is actually duplicate}).P(\text{$e_{m+1}$ is reported duplicate}) \nonumber\\
&= P(\text{$e_{m+1}$ is actually duplicate}).P(\text{all bit posotions in $H_{m+1}$} \nonumber \\
& \qquad \qquad\text{are $1$ when $e_{m+1}$ arrived}) \nonumber \\
&= (1-Y_{m+1}).X_{m+1}
\end{align}
\begin{align}		
DIS_{m+1}&= P(\text{$e_{m+1}$ is actually a distinct}).P(\text{$e_{m+1}$ is reported distinct}) \nonumber\\
&= P(\text{$e_{m+1}$ is actually a distinct}).P(\text{not all bit positions in} \nonumber \\
& \qquad \qquad \text{$H_{m+1}$ are $1$ when $e_{m+1}$ arrived}) \nonumber\\
&= Y_{m+1}.(1-X_{m+1})
\end{align}

We assume that elements of the stream are uniformly randomly drawn from a finite universe $\Gamma$, with $|\Gamma| = U$. \cite{rsbf} Then we can compute the value of $Y_{m+1}$, the probability that $e_{m+1}$ is a distinct element, as follows:
\begin{align}
Y_{m+1} = \left(\frac{U-1}{U}\right)^m
\end{align}
 
As $U-1 \leq U$, $Y_{m+1}$ tends to $0$ as the stream length $m$ tends to infinity. Hence naturally for any algorithm FPR tends to $0$ as the stream length increases. Intuitively this is true because the probability of an incoming element to be distinct decreases with time. However to ensure low FNR for large streams, $X_{m+1}$ must tend to $1$ as $m$ increases. We will show in the analysis of our various algorithms that all of them maintain this property. Hence we attain a very low FNR as well as very low FPR on large data streams.



\section{Biased Reservoir Sampling based Bloom Filter (BRSBF) Approach }
\subsection{BRSBF-I}
\label{sec:brsbf_1}
The design of BRSBF is motivated by the biased reservoir sampling technique for evolving stream \cite{charu}. The basic structure of BRSBF and RSBF are same but the insertion and deletion policies for an incoming data element are different. In BRSBF also we have $k$ bloom filters each of size $s$ bits. All bits are initially set to $0$. Each new data element of the stream is mapped to one of the $s$ bits in each of the $k$ bloom filter using $k$ uniform random hash function. If these $k$ bit positions are already set, then BRSBF declares this element as duplicate otherwise distinct.

Each time BRSBF declares an element $e_{i}$ of the stream as distinct, it inserts that element into the Bloom filters. As before, insertion of $e_i$ takes place by setting the $k$ bit positions corresponding to $e_i$ as $1$. In contrast, RSBF inserts a distinct element $e_i$, $i>s$ of the stream with a probability $p_i=s/i$. But inserting too many elements of the infinite stream into the Bloom filter will lead to high false positive rate. Hence each time we insert a new element in the Bloom filter, we reset some bits from the Bloom filter to $0$ in order to strike a balance between false positive rate and false negative rate. To be more precise, in BRSBF-I we uniformly randomly choose one bit from each of the $k$ Bloom filters and reset that bit to $0$. Note that, it might be possible that the chosen bit was already $0$. This helps in preventing too many elements getting deleted from the Bloom filters which in turn checks false negative rate from becoming high. In contrast, RSBF algorithm resets one bit from each of the $k$ Bloom filter every time an element was chosen to be inserted.

However from the stability perspective, the behavior of RSBF and BRSBF matches closely. In both of them, the insertion procedure selects $k$ random bits to be set to $1$ and deletion procedure selects $k$ random bits to be set to $0$. And each time insertion happens, deletion follows. Hence the both the approach leads to near constant number of $1$'s and $0$'s in the Bloom filter leading to stability. We have given theoretical proofs of this fact in later part of the paper.
 
One interesting aspect of the BRSBF algorithm is that it can capture the biased nature of the stream. TODO: More on this??

\begin{algorithm}[H]
\begin{center}
        \caption{$BRSBF-I(S)$}
        \label{algo:brsbf_algo}
        \begin{algorithmic}
                \REQUIRE Threshold FPR ($FPR_t$), Memory in bits ($M$), and Stream ($S$)
                \ENSURE Detecting \emph{duplicate} and \emph{distinct} elements in $S$

                \medskip

                \STATE Compute the value of $k$ from $FPR_t$.
                \STATE Construct $k$ Bloom filters each having $M/k$  bits of memory.
                \FOR{each element $e$ of $S$}
                        \STATE Hash $e$ into $k$ bit positions, $H={h_1,\cdots,h_k}$.
                        \IF{all bit at positions $H$ are set}
                        	\STATE $Result \gets DISTINCT$
						\ELSE
							\STATE $Result \gets DUPLICATE$
						\ENDIF

                        \IF{$e$ is DISTINCT}                      
								\STATE Randomly select k bit positions $hat{H}=\hat{h}_{1},\hat{h}_{2},...,\hat{h}_{k}$ one each from the $k$ Bloom filters.
								\STATE Reset all bits in $\hat{H}$ to $0$.	
							\STATE Set all the bits in $H$ to $1$.
						\ENDIF
                \ENDFOR
        \end{algorithmic}
\end{center}
\end{algorithm}

\subsection{BRSBF-II}
\label{sec:brsbf_2}
The second variation of the BRSBF algorithm, which we call BRSBF-II, differs from BRSBF-I in the way deletion from the Bloom filters take place. In BRSBF-I, whenever we insert an element $e_i$ into the Bloom filter we reset one bit from each of the $k$ Bloom filters. But in BRSBF-II, while deletion, we first randomly select one Bloom filter and then reset one bit from the selected Bloom filter. The rest of the algorithms are same.

Compared to BRSBF-I, BRSBF-II performs deletion in a conservative manner. This leads to very low FNR for BRSBF-II as the structure will remember signature of more elements compared to that BRSBF-I will remember. But on the flip side, since more elements are remembered, more elements are falsely reported as duplicate. Hence false positive rate increases. So for application which requires very low FNR, but can compromise with slightly higher FPR can adopt this version of the algorithm. We have proven theoretically and also have provided empirical results showing that the trade off between FPR and FNR of both the BRSBF algorithms are better paid off that their SBF counterpart.


\begin{algorithm}[H]
\begin{center}
        \caption{$BRSBF-II(S)$}
        \label{algo:brsbfII_algo}
        \begin{algorithmic}
                \REQUIRE Threshold FPR ($FPR_t$), Memory in bits ($M$), and Stream ($S$)
                \ENSURE Detecting \emph{duplicate} and \emph{distinct} elements in $S$

                \medskip

                \STATE Compute the value of $k$ from $FPR_t$.
                \STATE Construct $k$ Bloom filters each having $M/k$  bits of memory.
                \FOR{each element $e$ of $S$}
                        \STATE Hash $e$ into $k$ bit positions, $H={h_1,\cdots,h_k}$.
                        \IF{all bit at positions $H$ are set}
                        	\STATE $Result \gets DISTINCT$
						\ELSE
							\STATE $Result \gets DUPLICATE$
						\ENDIF

                        \IF{$e$ is DISTINCT}                      
                        	\STATE Randomly select a Bloom filter $B_{i}$
							\STATE Randomly select a bit $\hat{h}_{i}$ from the $B_{i}^{th}$ Bloom flter
							\STATE Reset $\hat{h}_{i}$ to $0$.		
							\STATE Set all the bits in $H$ to $1$.
						\ENDIF
                \ENDFOR
        \end{algorithmic}
\end{center}
\end{algorithm}

\subsection{Analysis of BRSBF-I}
To compute the probability of FPR or FNR at $e_{m+1}$, we need to compute $X_{m+1}$, the probability that all bit positions in $H_{m+1}$ are $1$ when $e_{m+1}$ arrived. Powered with the framework that we have built in the previous section, it'll immediately give us $FPR_{m+1}$ and $FNR_{m+1}$. So now we turn our focus on deriving $X_{m+1}$.

We have $e_{m+1}$, the $(m+1)^{th}$ element of the stream, hashing to $H_{m+1} = {h_1,h_2,...,h_k}$ positions, where each $h_i \in [1,s]$ for the $i^{th}$ Bloom filter. Initially all the bits of the Bloom filters are set to $0$. Since all the Bloom filters are identical and independent, first we will consider only one Bloom filter. Then we will extend our argument for $k$ Bloom filters. Let us assume $l$ is the last iteration when ${h}_{i}^{th}$ bit position of the $i^{th}$ Bloom filter goes from $0$ to $1$. Thereafter $h_i$ was never reset. A bit in the Bloom filter is reset by BRSBF-I only when some element is inserted. So $h_i$ will not be reset in an iterations $j$ ($l+1 \leq j \leq m$) if $e_j$ is not inserted (that is $e_j$ is reported as duplicate) or if $e_j$ is selected for insertion, then some other bit position is chosen to be reset. The probability of some other bit position to be chosen is $\left(1-\frac{1}{s}\right)$ Let us denote the probability of such a transition by $P_{trans}^{(l)}$. Hence,

\begin{align}
P_{trans}^{(l)}&= P(\text{$l$ is the last iteration when $h_{i}$ is set to $1$ thereafter it was never reset}) \nonumber \\
&=P(\text{$e_{l}$ was reported distinct}).P(\text{$e_l$ chooses $h_{i}$}).P(\text{$h_{i}$ was never reset thereafter}) \nonumber\\
&=P(\text{$e_{l}$ was reported distinct}).P(\text{$e_l$ chooses $h_{i}$}) \left\lbrace \prod_{i=l+1}^{m}\left[ P(\text{$e_{i}$ was reported duplicate}) \right. \right.\nonumber \\ 
& \qquad \left. \left. + P(\text{$e_{i}$ was reported distinct}).(1-\frac{1}{s})\right] \right\rbrace \nonumber\\
&=\left\lbrace(1-X_{l}).Y_{l} + (1-X_{l})(1-Y_{l})\right\rbrace.\frac{1}{s}.\left\lbrace \prod_{i=l+1}^{m}\left[X_{i}+(1-X_{i})(1-\frac{1}{s})\right]\right\rbrace
\end{align}

But we do not know $l$. Actually this transition can happen in any iteration from $1$ to $m$. Therefore, $l \in [1,m]$. Now this same analysis holds for all the $k$ Bloom filters similarly. Therefore we can write the expression for $X_{m+1}$ as follows:

\begin{align}
X_{m+1}&={\left[\sum_{l=1}^{m}\left\lbrace(1-X_{l}).Y_{l} + (1-X_{l})(1-Y_{l})\right\rbrace.\frac{1}{s}.\left\lbrace \prod_{i=l+1}^{m}\left[X_{i}+(1-X_{i})(1-\frac{1}{s})\right]\right\rbrace\right]}^{k} \nonumber \\
&={\left[\sum_{l=1}^{m}(1-X_{l}).\frac{1}{s}.\left\lbrace \prod_{i=l+1}^{m}\left[X_{i}+(1-X_{i})(1-\frac{1}{s})\right]\right\rbrace\right]}^{k}
\end{align}

Carefully observing the right hand side of the above equation, we can write the following recurrence relation for $X_{m+1}$:

\begin{align}
X_{m+1}&={\left[ {(X_{m})}^{\frac{1}{k}}\left\lbrace X_{m}+(1-X_{m}).(1-\frac{1}{s})\right\rbrace + (1-X_{m}).\frac{1}{s}\right] }^{k}
\end{align}

We show that $X$ is monotonically increasing until it converges to $1$. We recall from section \ref{framework} that:
\begin{align*}
FNR_{m+1}&= (1-Y_{m+1}).(1-X_{m+1})
\end{align*}
Hence our algorithm exhibits very low FNR with increasing stream length. Later we present empirical result to justify the claim that $X$ converges to $1$ and we also show that the convergence rate is fast.

\begin{theorem}
$X$ is monotonically increasing until it converges to $1$.
\end{theorem}
\begin{proof}
From equation no 4.9 [reference] we observe that:
\begin{align}
X_1 &= 0 \nonumber\\
X_2 &= \frac{1}{s^k} \nonumber
\end{align}
From equation no 4.10 [reference] we can write:
\begin{align*}
{\left(\frac{X_{m+1}}{X_m}\right)}^{\frac{1}{k}}&=X_{m}+(1-X_{m})(1-\frac{1}{s})+\frac{1}{X_{m}^{\frac{1}{k}}}.(1-X_{m}).\frac{1}{s} \\
&=1-(1-X_m).\frac{1}{s}+(1-X_m).\frac{1}{s.X_{m}^{\frac{1}{k}}} \\
&=1+(1-X_m).\frac{1}{s}.(X_{m}^{-\frac{1}{k}}-1)
\end{align*}

The second term on the right hand side is clearly positive when $X_m<1$. Therefore if $X_m < 1$, then $X_{m+1} > X_{m}$. If $X_m = 1$ then $X_{m+1} =1$. Therefore $X$ monotonically increases until it reaches $1$.
\end{proof}

\subsection{Analysis of BRSBF-II}

The FPR and FNR analysis of BRSBF-II is very similar to BRSBF-I. The only difference is in the way deletion of bits take place. In BRSBF-I whenever a new data element is inserted into the Bloom filters, one randomly chosen bit was reset from each of the Bloom filters. In BRSBF-II, after insertion we randomly select one Bloom filter and then randomly reset one bit from the selected Bloom filter. The probability that the bit $h_i$ (We are following the same convention as that of the section 4.3 ?? ) was not reset in an iteration in which some element was inserted is $\left( \frac{1}{k}.\left(1-\frac{1}{s}\right) + (1-\frac{1}{k}) \right)$ or $\left(1-\frac{1}{ks}\right)$. So we can write the expression for $X_{m+1}$ as follows:

\begin{align}
X_{m+1}&={\left[\sum_{l=1}^{m}(1-X_{l}).\frac{1}{s}.\left\lbrace \prod_{i=l+1}^{m}\left[X_{i}+(1-X_{i})(1-\frac{1}{ks})\right]\right\rbrace\right]}^{k}\\
&={\left[ {(X_{m})}^{\frac{1}{k}}\left\lbrace X_{m}+(1-X_{m}).(1-\frac{1}{ks})\right\rbrace + (1-X_{m}).\frac{1}{s}\right] }^{k}
\end{align}

X still remains monotonically increasing until it reaches $1$. To see this, we write the expression for $\frac{X_{m+1}}{X_{m}}$.
\begin{align*}
{\left(\frac{X_{m+1}}{X_m}\right)}^{\frac{1}{k}}&=X_{m}+(1-X_{m})(1-\frac{1}{ks})+\frac{1}{X_{m}^{\frac{1}{k}}}.(1-X_{m}).\frac{1}{s} \\
&=1+(1-X_m).\frac{1}{s}.(X_{m}^{-\frac{1}{k}}-\frac{1}{k})
\end{align*}
Since as long as $X_m<1$, the second term on the right hand side remains positive. Hence $X$ monotonically increases until it reaches $1$ following a similar argument as previous section.[reference]

\section{LBBRSBF}

In this section we will consider two more variation of the biased reservoir based sampling. We call them Load Balanced Biased Reservoir based SBF (LBBRSBF). In these variations we make the Bloom filters load balanced. This is achieved by performing load based deletions from the Bloom filters. This ensures stability in the Bloom filter structures by keeping the count of $0$ and $1$ almost constant. The two variations differs from each other in the way load distribution takes place. In the first variation, each Bloom filter is treated independently and deletion of a bit from a Bloom filter solely depends on the load of that Bloom filter. Hence each Bloom filter attains stability independently of each other. Whereas in the second variation the deletion decision is taken based on the load of the complete structure. Here the focus is on stability of the complete structure. Motivation?

\subsection{LBBRSBF-I}
In LBBRSBF-I, load (the number of bits set) in each of the Bloom filters is maintained by our algorithm. When an element $e$ is reported as distinct by the algorithm, we insert $e$ into the Bloom filters. Like before, this is done by setting the bits is $H$ to $1$. But instead of performing deterministic deletion from the Bloom filters, we perform randomized deletion from the Bloom filters. From each filter we first select a random bit position and then reset it with probability $L_{m+1}(i)/s$. $L_{m+1}(i)$ denotes the load of the $i^{th}$ Bloom filter when $e_{m+1}$ arrived. The detailed algorithm is given in \ref{algo:lbbrsbf_algo}.

This variation enforce stability in each of the Bloom filters. This in turn enforces low FPR and FNR. In one front we are preventing the number of set bits in each Bloom filter from becoming high. This reduces the FPR. On other side, we are performing load based deletion of bits from each of the Bloom filter which curbs down the FNR.


\begin{algorithm}[H]
\begin{center}
        \caption{$LBBRSBF-I(S)$}
        \label{algo:lbbrsbf_algo}
        \begin{algorithmic}
                \REQUIRE Threshold FPR ($FPR_t$), Memory in bits ($M$), and Stream ($S$)
                \ENSURE Detecting \emph{duplicate} and \emph{distinct} elements in $S$

                \medskip

                \STATE Compute the value of $k$ from $FPR_t$.
                \STATE Construct $k$ Bloom filters each having $M/k$  bits of memory.
                \FOR{each element $e$ of $S$}
                        \STATE Hash $e$ into $k$ bit positions, $H={h_1,\cdots,h_k}$.
                        \IF{all bit at positions $H$ are set}
                        	\STATE $Result \gets DISTINCT$
						\ELSE
							\STATE $Result \gets DUPLICATE$
						\ENDIF

                        \IF{$e$ is DISTINCT}                      
                        	\FORALL{Bloom filter $B_{i}$}
                        		\STATE Select a random bit position $\hat{h_{i}}$.
                        		\STATE Reset $\hat{h_{i}}$ with probability $L(i)/s$ where $L(i)$ is the number of ones in the Bloom filter $B_{i}$.
                        	\ENDFOR
							\STATE Set all the bits in $H$ to $1$.
						\ENDIF
                \ENDFOR
        \end{algorithmic}
\end{center}
\end{algorithm}

\subsection{LBBRSBF-II}
In LBBRSBF-II, we maintain the total load of the structure (total no of set bits in the structure). When the current element of the stream,$e_{m+1}$ , is reported as distinct, the algorithm inserts $e_{m+1}$ into the structure. It then decide to perform deletion from the Bloom filter with probability $L/ks$ where $L$ is the total load of the Bloom filters. If deletion decision is taken, then from each of the $k$ Bloom filters one random bit is selected and reset to $0$. The detailed algorithm is given in \ref{algo:lbbrsbfII_algo}.

May be add more?

\begin{algorithm}[H]
\begin{center}
        \caption{$LBBRSBF-II(S)$}
        \label{algo:lbbrsbfII_algo}
        \begin{algorithmic}
                \REQUIRE Threshold FPR ($FPR_t$), Memory in bits ($M$), and Stream ($S$)
                \ENSURE Detecting \emph{duplicate} and \emph{distinct} elements in $S$

                \medskip

                \STATE Compute the value of $k$ from $FPR_t$.
                \STATE Construct $k$ Bloom filters each having $M/k$  bits of memory.
                \FOR{each element $e$ of $S$}
                        \STATE Hash $e$ into $k$ bit positions, $H={h_1,\cdots,h_k}$.
                        \IF{all bit at positions $H$ are set}
                        	\STATE $Result \gets DISTINCT$
						\ELSE
							\STATE $Result \gets DUPLICATE$
						\ENDIF

                        \IF{$e$ is DISTINCT}   
							\STATE Decide with probability $L/k.s$ whether to perform deletion or not. L is the total no of ones in the $k$ Bloom filters.	
                        	\IF {Deletion should be performed}
                        		\FORALL{Bloom filter $B_{i}$}
              		          		\STATE Select a random bit position $\hat{h_{i}}$ and reset it to $0$.
              		          	\ENDFOR
                        	\ENDIF
							\STATE Set all the bits in $H$ to $1$.
						\ENDIF
                \ENDFOR
        \end{algorithmic}
\end{center}
\end{algorithm}

\subsection{Analysis of LBBRSBF-I}

To compute the probability of FNR and FPR of LRSBF-I, we also need to find the expected load of the Bloom filters at any iteration. Let $L_{m+1}^{i}$ denotes the expected no of bits set in the $i^{th}$ Bloom filter when $e_{m+1}$ arrived. So we have the following scenario: $e_{m+1}$ hashes to $h_i$ bit position of the $i^{th}$ Bloom filter. We are interested in finding out the probability of $h_i$ being already set to $1$ for all $i \in [1,k]$. This will give us $X_{m+1}$ and which in turn will give us FPR and FNR. 

Now as similar to our earlier arguments [reference], we assume that $l$ is the last iteration when $h_i$ was set to $1$ and after that it was never reset. $h_i$ will not be reset in an iteration $j(l+1\leq j \leq m)$ if one the following happens: (i) $e_j$ was reported as duplicate and hence not inserted into the Bloom filter, (ii) $e_j$ was inserted into the Bloom filter and with probability $1-\frac{L_{m+1}^{i}}{s}$ no bits were reset from $i^{th}$ Bloom filter, (iii) $e_j$ was inserted into the Bloom filter and with probability $\frac{L_{m+1}^{i}}{s}$ deletion from $i^{th}$ Bloom filter was decided, but some bit other than $h_i$ was chosen for deletion with probability $\left(1-\frac{1}{s}\right)$. This same argument applies to all the $k$ bloom filters. Also $l$ can vary from $1$ to $m$.

Therefore following the LBRSBF-I algorithm we write the expression for $X_{m+1}$ as follow:

\begin{align}
X_{m+1}&=P(\text{all bit positions in $H_{m+1}$ are $1$ when $e_{m+1}$ arrived}) \nonumber\\
&={\left[\sum_{l=1}^{m}P(\text{$l$ is the last iteration when $h_i$ is set to $1$, thereafter it was never reset}) \right]}^k\nonumber \\
&={\left[\sum_{l=1}^{m}P(\text{$e_l$ was reported distinct}).P(\text{$e_l$ chooses $h_i$}).P(\text{$h_i$ was never reset thereafter}) \right]}^k\nonumber \\
&={\left[\sum_{l=1}^{m}(1-X_{l}).\frac{1}{s}.\left\lbrace \prod_{i=l+1}^{m}\left[X_{i}+(1-X_{i})\left((1-\frac{L_{m+1}^{i}}{s})+\frac{L_{m+1}^{i}}{s}(1-\frac{1}{s})\right)\right]\right\rbrace\right]}^{k} \nonumber\\
&={\left[\sum_{l=1}^{m}(1-X_{l}).\frac{1}{s}.\left\lbrace \prod_{i=l+1}^{m}\left[X_{i}+(1-X_{i})(1-\frac{L_{m+1}^{i}}{s^2})\right]\right\rbrace\right]}^{k} \\
&={\left[ {(X_{m})}^{\frac{1}{k}}\left\lbrace X_{m}+(1-X_{m}).(1-\frac{L_{m+1}^{i}}{s^2})\right\rbrace + (1-X_{m}).\frac{1}{s}\right] }^{k}
\end{align}

Now we need to find out the expected load $L_{m+1}^{i}$ of the $i^{th}$ Bloom filter at the time when $e_{m+1}$ arrived. Let us associate an indicator random variable $I_j$ with each bit $j$ of the Bloom filters. $I_j$ is $1$ if $j$ is $1$ otherwise $0$. Also let $Z^{i}$ be random variable such that $Z^{i}=\sum_{j=1}^{s}I_j$. Therefore $E[Z^{i}]$ will give us the expected load of the $i^{th}$ Bloom filter.
\begin{align}
L_{m+1}^{i}&=E[Z^{i}]\nonumber \\
&=\sum_{j=1}^{s}E[I_j] \nonumber \\
&=\sum_{j=1}^{s}P(\text{$j^{th}$ bit was set to 1 when $e_{m+1}$ arrived}) \nonumber \\
\end{align}



